Learning to Participate through Trading of Reward Shares

Enabling autonomous agents to act cooperatively is an important step to integrate artificial intelligence in our daily lives. While some methods seek to stimulate cooperation by letting agents give rewards to others, in this paper we propose a method inspired by the stock market, where agents have the opportunity to participate in other agents' returns by acquiring reward shares. Intuitively, an agent may learn to act according to the common interest when being directly affected by the other agents' rewards. The empirical results of the tested general-sum Markov games show that this mechanism promotes cooperative policies among independently trained agents in social dilemma situations. Moreover, as demonstrated in a temporally and spatially extended domain, participation can lead to the development of roles and the division of subtasks between the agents.

==> content/0-introduction.tex <==
\section{Introduction}
Coordinating multiple agents to behave in the interest of all agents is often difficult to implement. In a simple decentralized model, agents tend to only optimize their own rewards without considering the effect of their actions on other agents. This type of optimization may lead to sub-optimal outcomes such as in the prisoner's dilemma or public good games. In more complex games, the agents’ risk-aversion as well as information asymmetry additionally deteriorate the likelihood of a desired outcome \cite{bargaining}. In several publications \cite{bucsoniu2010multi}, this problem is tackled by using reinforcement learning. An agent can punish or reward the other agents depending on the effect of their chosen actions on their own rewards. By punishing and/or rewarding over multiple episodes, the agents learn to include other agents' rewards in their optimization problem. My contribution to the multi-agent framework is to substitute punishments and rewards by a market, in which agents are allowed to trade their shares in other agents' rewards. This market may lead to a ``better'' equilibrium by letting agents directly participate in other agents' rewards. Precisely, a ``socially optimal'' equilibrium may be established due to the direct incorporation of all global rewards instead of only incorporating individual rewards. Enabling the agents to trade their shares at a fair price, while at the same time creating a trading path that in fact leads to a beneficial distribution of shares, is the most challenging implementation in this model. 
I let the agents exchange their shares in equal amounts without the need of prices. But I also test alternatives. Namely, the agents could decide to participate in a common reward pool, or the joint individual rewards could just be divided among the agents. As a next step, I suggest introducing a broker that sets prices such that agents end up with the ``market portfolio'', a portfolio that mirrors the whole ``market'' consisting of all agents. The intuition behind the ``market portfolio'' is derived from financial stock portfolios. Following this intuition, an external market broker could be regarded as a market-maker.

% -------------------------------------------------------------------------------- %

There are advantages of using direct participation in other agents' rewards through trading shares. In another model \cite{lio}, agents learn a ``socially optimal behavior'' through an incentive function. In my suggested model, agents instead learn through their market participation. Firstly, the incorporation of a market seems to be an intuitive solution to establish a trading path to a ``new'' equilibrium. Secondly, agents do not have to incentivize other agents via punishment or reward transactions. These transactions may be costly and may only be rational in the long run, but not for single periods. Thus, agents are required to have perfect foresight to justify the transactions. Additionally, the amount of transactions seems random. In a market model, prices could be dynamic according to the saying ``the market knows best''. Furthermore, equilibria may even adapt to changing rewards. A market model does not necessarily need this foresight. Moreover, the path to the new equilibrium could potentially include fewer distortions. Lastly, the incentivizing transactions do not stop. In my suggested model, agents only trade if they receive a benefit from it.

% -------------------------------------------------------------------------------- %

Broadly, this research analyzes the welfare effects of letting agents trade shares in their returns. Market participation might make agents worse/better off, improve distributional problems of (naïve/sophisticated) agents, solve match making via closeness and work well with many agents.

% -------------------------------------------------------------------------------- %

I first provide background information in the form of preliminaries (\autoref{sec:prelimiaries}) and related literature (\autoref{sec:relatedwork}). In the main section of this work (\autoref{sec:participate}), I first motivate why market participation may be beneficial. Then, I analyze a simple prisoner's dilemma and show that the outcome could improve through participation in the market. Since the market participation should also be beneficial in dynamic, more complex dilemmas, I also study the effects of participation in the clean-up game. For this game, I also shed light on the question whether participation can enable cooperation in the case of more than two agents. I end my work with a conclusion and a brief outlook on potential future research (\autoref{sec:conclusion}). The code
for the experiments in this paper can be found on github\footnote{\url{https://github.com/TimMatheis/Learning-to-participate}}.
